The Parametric Stability of Well-separated Spherical Gaussian Mixtures

We quantify the parameter stability of a spherical Gaussian Mixture Model (sGMM) under small perturbations in distribution space. Namely, we derive the first explicit bound to show that for a mixture of spherical Gaussian $P$ (sGMM) in a pre-defined model class, all other sGMM close to $P$ in this model class in total variation distance has a small parameter distance to $P$. Further, this upper bound only depends on $P$. The motivation for this work lies in providing guarantees for fitting Gaussian mixtures; with this aim in mind, all the constants involved are well defined and distribution free conditions for fitting mixtures of spherical Gaussians. Our results tighten considerably the existing computable bounds, and asymptotically match the known sharp thresholds for this problem.

==> sphgmm-alg.tex <==
\section{Evaluating Good Fit of Mixtures of Spherical Gaussians}
\hanyuz{This is an unfinished section. Major techniques are same. But I think it is not urgent to complete this as the previous theorem shold be tested first on some real datasets.}

\newcommand{\deltamu}{\delta^{\mu}}
\newcommand{\deltaeta}{\delta^{\eta}}
\newcommand{\deltapi}{\delta^\pi}
\label{sec:alg}
For an arbitrary distribution $Q$, suppose we have find a good fit $P=\sum_{k=1}^K\pi_kN_d(\mu_k,\sigma_k^2I_d)$ to $Q$ within total variation distance $\epsilon$. If this fit is well separated by at least $c_0\eta_0$ and has a minimal component proportion $\pi_{\min}$, previous result shows that, any other good fit $P'$ to $Q$ that lies in the model class $\mathcal{M}(K,\pi_{\min},c)$ is component-wise close to $P$. On the other hand, given the much information provided by $P$, as its parameters are known, upper bounds can be obtained specific to each components.

We start by introducing some notations. Since all parameters in $P$ is known, it will be helpful to use specific separation parameters. Define
\begin{equation}
    s_{ij}=\frac{\norm{\mu_i-\mu_j}}{\sigma_i+\sigma_j}\;.
\end{equation}
The previous \theoremref{thm:main1} shows that, if $\min_{i\neq j}s_{ij}\geq c > c_0\eta_0$, then $P$ and $P'$ are componentwise close through upper bounds for each pair of corresponding components $P_i,P_i'$ of 
\begin{align}
    \deltamu_{i}&:=\frac{\norm{\mu_i-\mu_i'}}{\max\{\sigma_i,\sigma_i'\}}\leq c^*\;, \\
     \deltaeta_{i} &:=  \max\{\frac{\sigma_i}{\sigma_i'},\frac{\sigma_i'}{\sigma_i}\}\leq  \eta^*\;,\\
     \deltapi_{i} &:=|\pi_i-\pi_i'|\leq 2\epsilon+K[1-(K-1)\pi_{\min}]\Phi(-C(c,c^*,\eta^*))\;.
\end{align}

In fact by utilizing the information given in $P$, we are able to compute data specific guarantee. 



==> sphgmm-exp.tex <==
\section{Examples}
\label{sec:exp}
Now we show some numerical examples of the main result. We shall show the stability bounds in some cotaminated distribution cases. Suppose there is an oracle distribution $P_0$ and $\tilde{P}_*=(1-\lambda)P_0+\lambda Q$ is the perturbed distribution. We shall show our stability bounds of using $P_0$ to fit $\tilde{P}_*$ by considering infinite sample size as a proof of concept. We shall show that when $\lambda$ is large enough, we can detect the misspecification as the stability guarantee will fail. In the following cases the global goodness of fit, measured by the distance between the principal spaces is zero. We compute the value $\epsilon$, the componentwise total variation distance, and plug it into the upper bound provided by \theoremref{thm:main1}. This total variation distance is computed by monte carlo simulation.\\

\noindent{\textbf{Example 1: two clusters in two dimension}}
First we consider $P_0=\frac{1}{2}N_2(\theta_1,\sigma^2 I_2)+\frac{1}{2}N_2(\theta_2,\sigma^2I_2)$ with
$$
\theta_1 = (-1,-\frac{2\sqrt{3}}{3}),\quad \theta_2 = (1,-\frac{2\sqrt{3}}{3})
$$
The contamination distribution is $N_2(\theta_3,\sigma^2 I)$ where $\theta_3 = (0,4\sqrt{3}/3)$. The result for this example is displayed in \figureref{fig:simplecase}. The results show that when $\lambda$ is as large as 0.1, we cannot get any meaningful upper bound. Thus it suggests that the fitting model may not be appropriate. Secondly, we observe that when $\lambda$ is small and $\epsilon$ between original fit and distribution is small, the probability parameter $\alpha$ will dominate the upper bound. These also explains that the bound is not quite useful when $\sigma=0.2$ since the separation is not large enough. 

\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/alphaVSsigma-ori2.png}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/epsilonVSsigma-ori2.png}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/ubVSsigma-ori2.png}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/dfMeanVSsigma-ori2.png}
    \end{minipage}
    \caption{Results on fitting two clusters in two dimension. 
    \textbf{Topleft:} How the probability parameter $\alpha$ changes with respect to $\sigma$.
    \textbf{Topright:} Computed TV distance of each component of $P_0$ fit with respect to $\sigma$.
    \textbf{Bottomleft:} Computed upper bound on TV distance between an arbitrary fit and $P_0$ with respect to $\sigma$.
    \textbf{Bottomright:} The maximum difference between the center parameter of each component and an arbitrary "good" fit with respect to $\sigma$. This type of upper bound cannot be derived when the total variation distance upper bound is larger than 0.5.}
    \label{fig:simplecase}
\end{figure}

\noindent{\textbf{Example 2: more clusters in higher dimension}}
Consider $P_0=\sum_{k=1}^K\frac{1}{K}P_k$ where each $P_k=N_d(\mu_k,I_d)$. The number of components $K$ is 2 or 5. Let $e_k$ be the vector with only the $k-$th entry being nonzero and one. 
$$
\mu_k = se_k,\sigma_k=\sigma_0=1
$$
Under this setting, the separation between each two mean is given by $s\sqrt{2}$. And the mean of $P_0$ is $\overline{\mu}=\frac{s}{K}\sum_{k=1}^Ke_k$. The perturbed distribution is $P_*=(1-\lambda)P_0+\lambda Q$. We consider two scenarios. (i) $Q$ is a background noise. Set $Q=N_d(\overline{\mu},100\sigma_0^2)$ (ii) $Q$ is an outlier. Set $Q=N_d(K\overline{\mu},0.01\sigma_0^2)$. Figure \figureref{fig:eg2bignoise} and \figureref{fig:eg2smallnoise} shows the computed total variation distance upper bound of these two cases. We can see that the bound is almost meaningless when $K$ is only moderately as large as five except when the separation is very large. 

\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/UpperBoundVSsigma-K=2-sigmasmall-0.png}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/UpperBoundVSsigma-K=5-sigmasmall-0.png}
    \end{minipage}
    \caption{Total variation distance upper bound for $Q = N_d(\overline{\mu},100\sigma_0^2I_d)$.}
    \label{fig:eg2bignoise}
\end{figure}

\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/UpperBoundVSsigma-K=2-sigmasmall-1.png}
    \end{minipage}
    \begin{minipage}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/UpperBoundVSsigma-K=5-sigmasmall-1.png}
    \end{minipage}
    \caption{Total variation distance upper bound for $Q = N_d(K\overline{\mu},0.01\sigma_0^2I_d)$.}
    \label{fig:eg2smallnoise}
\end{figure}




==> sphgmm-tech.tex <==

In this section we identify the key technical tools used in the proof of our main result, some of which can be of independent interest. All the proofs can be found in \sectionref{sec:proof-main} in supplementary materials. 

\paragraph{Total Variation Distance Between Spherical Gaussians}
We develop a lemma upper bounding parameter distances between
spherical Gaussians given their total variation distance. For this, one can use
Hellinger distance, which includes an anlytical expression as a
natural lower bound \citep{Gibbs2002probDist}, but they are usually not
tight in constants and therefore they cannot separate the bound in
mean parameter and variance parameter. \citet{devroye2020total}
proposes another lower bound starting from the definitions but their results are
only meaningful when the total variation distance is sufficiently
small.
%
\begin{lemma}
  \label{lem:GaussianTV}
  Suppose $P_1 = N_d(\mu_1,\sigma_1^2 I_d)$ and $P_2 = N_d(\mu_2,\sigma_2^2 I_d)$. Let $C_0(\rho)=2\Phi^{-1}(1-\frac{\rho}{2})$ and $\eta_0(\rho)$ be the solution of
   \begin{equation}
    1-\rho = F_d\left(\frac{2\eta^2 \log \eta}{\eta^2-1}\right) - F_d\left(\frac{2 \log \eta}{\eta^2-1}\right)\;.
  \end{equation}
  Then the following holds:
  \begin{itemize}
    \item If $\norm{\mu_1-\mu_2}\geq C_0(\rho)(\sigma_1+\sigma_2)/2$, then $TV(P_1,P_2)\geq 1-\rho$. Equality holds iff $\sigma_1 = \sigma_2$ and $\norm{\mu_1-\mu_2} = C_0(\rho)(\sigma_1+\sigma_2)/2$.
    \item If $\max\{\sigma_1/\sigma_2,\sigma_2/\sigma_1\}\geq \eta_0(\rho)$, then $TV(P_1,P_2)\geq 1-\rho$. Equality holds iff $\mu_1 = \mu_2$ and $\max\{\sigma_1/\sigma_2,\sigma_2/\sigma_1\} = \eta_0(\rho)$.
  \end{itemize}
\end{lemma}

\paragraph{Component-wise Comparisons in Mixture Models}
The second key ingredient for proving our result is a group of
component-wise comparison lemmas on two mixture distributions with
small total variation distance. In the following lemmas, consider two
mixture distributions $P=\sum_{i=1}^K \pi_i P_i$ and
$P'=\sum_{j=1}^{K'} \pi_j' P_j$ and denote $\pi_{\min} =
\min_{i,j}\{\pi_i,\pi_j'\}$ and
$\pi_{\max}=\max_{i,j}\{\pi_i,\pi_j'\}$.  The proofs can be found in
\sectionref{sec:proof-main}; these lemmas essentially show that (1)
the weighted sum of component-wise total variation difference is upper
bounded if the two mixtures are close and (2) when two well-separated
mixtures have same number of components, under particular
correspondence conditions, their mixture proportions are close.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lemma: component-wise-tv
\begin{lemma}
  \label{lem:component-wise-tv-P}
  Suppose $TV(P,P')\leq 2\epsilon$. For any $j\in[K']$, if there exists a collection of sets $\{A_{ij}\}_{i\in[K]}$ such that $\rho_{ij}=1-P_i(A_{ij})+P_j'(A_{ij})\in [0,1]$ for all $i\in[K]$, then
   \begin{equation}
   \sum_{i=1}^K\max\{\pi_i,\pi_j'\}\rho_{ij}\geq \pi_j'-2\epsilon\;,\quad\sum_{i=1}^K \pi_i\rho_{ij}\geq \pi_{\min}-2\epsilon\;.
   \label{eq:component-wise-tv-P}
   \end{equation}
   Similarly, if there exists a collection of sets $\{B_{ij}\}_{i\in[K]}$ such that $\rho_{ij}=1-P_j'(B_{ij})+P_i(B_{ij})\in [0,1]$ for all $i\in[K]$, equation \label{eq:component-wise-tv-P2} also holds.
\end{lemma}
%      
This lemma stems from the fact that there cannot be a set that has a
large probability mass of a component in $P_i$ of $P$ but has small
probability mass from every component $P'_j$ of $P'$. $A_{ij}$ is the set that has a large probability mass under $P_i$ but small under $P_j'$, while $B_{ij}$ vice versa. A symmetric result can be obtained by switching the role of $P$ and $P'$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lemma: rho1 rho2

\lemmaref{lem:component-wise-tv-P} is particularly useful when,
for some component $P_j'$, all components $P_i,\,i\neq j$ are far away from $P_j'$ in total variation distance; then by \lemmaref{lem:component-wise-tv-P} one can
upper bound the total variation distance between $P_j'$ and the
remaining component $P_j$ of $P$.
%
\begin{lemma}
  Suppose $TV(P,P')\leq 2\epsilon$ and denote $\pi_{\min} = \min_{i,j}\{\pi_i,\pi_j'\}$.\comment{ Further suppose $\max\{K,K'\}\leq 1/\pi_{\min}$ and $\max\{K,K'\}\leq 1/\pi_{\min}$.} Consider two components $P_{j_0},P_j'$ with $\pi_{j_0}\leq \pi_{j}'$. If for all $i\in[K],i\neq j_0$, there is a set $A_{ij}$ such that $P_i(A_{ij})-P_j'(A_{ij}) \geq 1-\rho$ with some constant $\rho$ satisfying
 $0\leq \rho \leq (\pi_{\min}-2\epsilon)/(1-\pi_{\min})$, it holds that
 \begin{equation}
 TV(P_{j_0},P_j') \leq \frac{2\epsilon}{\pi_{\min}}+\frac{1-\pi_{\min}}{\pi_{\min}}\rho\;.
 \label{eq:tv-bound-unknown-pi}
 \end{equation}
 \label{lem:rho1-rho2}
\end{lemma}
%
Now, we obtain a component-wise comparison result for the differences in mixture proportions between corresponding components. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
  \label{lem:diff-proportion}
  Suppose $TV(P,P')\leq 2\epsilon$. Denote $\pi_{\min} = \min_{i,j}\{\pi_i,\pi_j'\}$ and $\pi_{\max} = \max_{i,j}\{\pi_i,\pi_j'\}$  If there is a pair of components $P_i,P_i'$ and a set $A$ such that for some $\rho\in (0,1)$, $\min\{P_i(A),P_i'(A)\}\geq 1-\rho$ and $\max_{j\neq i}\{P_j(A),P_j'(A)\} \leq \rho$, then
  \begin{equation}
    |\pi_i-\pi_i'|\leq 2\epsilon + (1+\pi_{\max}-\pi_{\min})\rho
  \end{equation}
\end{lemma}


